SHARE: Single-view Human Adversarial REconstruction

The accuracy of 3D Human Pose and Shape reconstruction (HPS) from an image is progressively improving. Yet, no known method is robust across all image distortion. To address issues due to variations of camera poses, we introduce SHARE, a novel fine-tuning method that utilizes adversarial data augmentation to enhance the robustness of existing HPS techniques. We perform a comprehensive analysis on the impact of camera poses on HPS reconstruction outcomes. We first generated large-scale image datasets captured systematically from diverse camera perspectives. We then established a mapping between camera poses and reconstruction errors as a continuous function that characterizes the relationship between camera poses and HPS quality. Leveraging this representation, we introduce RoME (Regions of Maximal Error), a novel sampling technique for our adversarial fine-tuning method. The SHARE framework is generalizable across various single-view HPS methods and we demonstrate its performance on HMR, SPIN, PARE, CLIFF and ExPose. Our results illustrate a reduction in mean joint errors across single-view HPS techniques, for images captured from multiple camera positions without compromising their baseline performance. In many challenging cases, our method surpasses the performance of existing models, highlighting its practical significance for diverse real-world applications.

==> figures/cyclical_error.tex <==
\begin{figure*}[t]
    \centering
    \vspace*{-1em}
    \begin{subfigure}{.5\textwidth}
    \includegraphics[width=\columnwidth]{images/resized_analysis_fig.pdf}
    \vspace*{-0.5em}
    \caption{\textbf{Sensitivity analysis on PARE with respect to camera pose} }
    \vspace*{-1em}
    % \label{fig:cyclical_errors}
    \end{subfigure}
    \begin{subfigure}{.4\textwidth}
    \includegraphics[height=2.7in,width=1.1\columnwidth]{images/re_sized_loss_landscape_pare.pdf}
    \vspace*{-0.5em}
    \caption{\textbf{Loss Landscape for PARE}}
    \vspace*{-1em}
    % \label{fig:loss_landscape}
    \end{subfigure}
    \caption{(a) \textbf{Sensitivity analysis on PARE with respect to camera pose using PA-MPJPE} The x-axis iterates through all camera poses $(\theta,\phi)$, where $\phi$ represents the azimuthal angle around the body (0, 360), and $\theta$ represents the vertical viewing angle (-60, 60) for each $\phi$. The y-axis represents the average error in PA-MPJPE over a diverse dataset encompassing a wide range of bodies, body poses, and environments. This plot explicitly depicts the average error associated with each camera pose, revealing a discernible oscillatory bias with varying performance in different regions around the human body. \\
    Figure 3. (b) \textbf{Loss Landscape for PARE.} The x-axis represents the scaled $\theta$ values, while the y-axis represents the scaled $\phi$ values, the z-axis depicts the predicted PA-MPJPE associated with a given camera pose. Additional plots for single-person datasets and comparisons with other HPS techniques are available in the appendix.}
\end{figure*}


